Analysis and Mitigations of Reverse Engineering Attacks on Local Feature Descriptors

As autonomous driving and augmented reality evolve, a practical concern is data privacy. In particular, these applications rely on localization based on user images. The widely adopted technology uses local feature descriptors, which are derived from the images and it was long thought that they could not be reverted back. However, recent work has demonstrated that under certain conditions reverse engineering attacks are possible and allow an adversary to reconstruct RGB images. This poses a potential risk to user privacy. We take this a step further and model potential adversaries using a privacy threat model. Subsequently, we show under controlled conditions a reverse engineering attack on sparse feature maps and analyze the vulnerability of popular descriptors including FREAK, SIFT and SOSNet. Finally, we evaluate potential mitigation techniques that select a subset of descriptors to carefully balance privacy reconstruction risk while preserving image matching accuracy; our results show that similar accuracy can be obtained when revealing less information.

==> figures/invsfm_comparison.tex <==
\begin{figure*}[t]
     \centering
     \begin{subfigure}
         \includegraphics[width=0.13\linewidth]{figures/invsfm_comparison/invsfm_test1.png}
     \end{subfigure}%
     \begin{subfigure}
         \includegraphics[width=0.13\textwidth]{figures/invsfm_comparison/invsfm_depth_result1.png}
     \end{subfigure}%
     \begin{subfigure}
         \includegraphics[width=0.13\textwidth]{figures/invsfm_comparison/invsfm_depth_sift_result1.png}
     \end{subfigure}%
     \begin{subfigure}
         \includegraphics[width=0.13\textwidth]{figures/invsfm_comparison/invsfm_depth_sift_rgb_result1.png}
     \end{subfigure}%
     \begin{subfigure}
         \includegraphics[width=0.13\textwidth]{figures/invsfm_comparison/invsfm_test1/sift_1200.png}
     \end{subfigure}%
     \begin{subfigure}
         \includegraphics[width=0.13\textwidth]{figures/invsfm_comparison/invsfm_test1/freak_1200.png}
     \end{subfigure}%
     \begin{subfigure}
         \includegraphics[width=0.13\textwidth]{figures/invsfm_comparison/invsfm_test1/sos_1200.png}
     \end{subfigure}
     
     \centering
     \begin{subfigure}
         \includegraphics[width=0.13\linewidth]{figures/invsfm_comparison/invsfm_test5.png}
     \end{subfigure}%
     \begin{subfigure}
         \includegraphics[width=0.13\textwidth]{figures/invsfm_comparison/invsfm_depth_result5.png}
     \end{subfigure}%
     \begin{subfigure}
         \includegraphics[width=0.13\textwidth]{figures/invsfm_comparison/invsfm_depth_sift_result5.png}
     \end{subfigure}%
     \begin{subfigure}
         \includegraphics[width=0.13\textwidth]{figures/invsfm_comparison/invsfm_depth_sift_rgb_result5.png}
     \end{subfigure}%
     \begin{subfigure}
         \includegraphics[width=0.13\textwidth]{figures/invsfm_comparison/invsfm_test5/sift_1200.png}
     \end{subfigure}%
     \begin{subfigure}
         \includegraphics[width=0.13\textwidth]{figures/invsfm_comparison/invsfm_test5/freak_1200.png}
     \end{subfigure}%
     \begin{subfigure}
         \includegraphics[width=0.13\textwidth]{figures/invsfm_comparison/invsfm_test5/sos_1200.png}
     \end{subfigure}
     
     \centering
     \begin{subfigure}
         \includegraphics[width=0.13\linewidth]{figures/invsfm_comparison/invsfm_test12.png}
     \end{subfigure}%
     \begin{subfigure}
         \includegraphics[width=0.13\textwidth]{figures/invsfm_comparison/invsfm_depth_result12.png}
     \end{subfigure}%
     \begin{subfigure}
         \includegraphics[width=0.13\textwidth]{figures/invsfm_comparison/invsfm_depth_sift_result12.png}
     \end{subfigure}%
     \begin{subfigure}
         \includegraphics[width=0.13\textwidth]{figures/invsfm_comparison/invsfm_depth_sift_rgb_result12.png}
     \end{subfigure}%
     \begin{subfigure}
         \includegraphics[width=0.13\textwidth]{figures/invsfm_comparison/invsfm_test12/sift_1200.png}
     \end{subfigure}%
     \begin{subfigure}
         \includegraphics[width=0.13\textwidth]{figures/invsfm_comparison/invsfm_test12/freak_1200.png}
     \end{subfigure}%
     \begin{subfigure}
         \includegraphics[width=0.13\textwidth]{figures/invsfm_comparison/invsfm_test12/sos_1200.png}
     \end{subfigure}
     
\caption{Left to Right: Ground truth image, results from~\cite{invsfm} using depth, depth+SIFT descriptors, and depth+SIFT+RGB to reconstruct the image, and our reconstructions using only SIFT, FREAK, or SOSNet descriptors.} 
\label{fig:invsfm_comparison}

\end{figure*}

==> figures/related_work_comparison.tex <==
\begin{figure*}[t]
\centering
     \begin{subfigure}[t]{0.23\textwidth}
         \includegraphics[align=c, width=\linewidth]{figures/related_work_comparison/ground_truth.png}
         \caption{Original} 
     \end{subfigure}\hspace*{1mm}
     \begin{subfigure}[t]{0.23\textwidth}
         \includegraphics[align=c, width=\textwidth]{figures/related_work_comparison/plaza_sift.png}
         \caption{Ours-SIFT\label{fig:ours_sift}} 
     \end{subfigure}\hspace*{1mm} 
    \begin{subfigure}[t]{0.23\textwidth}
         \includegraphics[align=c, width=\linewidth]{figures/related_work_comparison/plaza_freak.png}
         \caption{Ours-FREAK} 
     \end{subfigure}\hspace*{1mm}
     \begin{subfigure}[t]{0.23\textwidth}
         \includegraphics[ align=c, width=\textwidth]{figures/related_work_comparison/plaza_sosnet.png}
         \caption{Ours-SOSNet}
     \end{subfigure}% 

     \begin{subfigure}[t]{0.30\textwidth}
         \includegraphics[width=\textwidth]{figures/related_work_comparison/plaza_weinzaepfel2011.jpg}
         \caption{\protect\citesupp{weinzaepfel2011reconstructing}-SIFT\label{fig:weinz_sift}}
     \end{subfigure}\hspace*{1mm}%
     \begin{subfigure}[t]{0.30\textwidth}
         \includegraphics[width=\textwidth]{figures/related_work_comparison/plaza_deangelo-brief-fast-p32.jpg}
         \caption{\protect\citesupp{d2013bits}-binary\label{fig:deangelo}}
     \end{subfigure}\hspace*{1mm}%
     \begin{subfigure}[t]{0.30\textwidth}
         \includegraphics[width=\textwidth]{figures/related_work_comparison/plaza_dosovitskiy.png}
         \caption{\protect\citesupp{dosovitskiy2016inverting}-SIFT\label{fig:dosovitskiy}}
     \end{subfigure} 
     \vspace{-2mm}
    \caption{(a) Original image and our reconstructions from SIFT (b), FREAK (c), and SOSNet (d) descriptors. Reconstructions by prior work from SIFT descriptors in~\protect\citesupp{weinzaepfel2011reconstructing} (e), and BRIEF descriptors in~\protect\citesupp{d2013bits} (f), and SIFT descriptors in~\protect\citesupp{dosovitskiy2016inverting} (g).
    % \ei{Why do we not show InvSfM in this figure?}
    }
    \label{fig:related_work_comparison}
\end{figure*}
